Superfluous Physics

A superweapon of modern physics superscribes a wide superset of phenomena, ranging from supernumerary rainbows to superfluidity and even possible supermultiplets.

==> section/super.tex <==
\section{SUPER}
Here's a super long list of `super-'-prefixed words.

marsupial
superabsorbent
superabundance
superaligned
superalimentation
supercilious
supercontinent
superdeluxe
superette
super expensive
super fast
superfluid
superhardened
superintendant
superjumbo
superlunar[y]
supermicros
superposable
supers
supersecret
superstore
supersweet
supinate
supine

Here's a list of other potentially-includable words:

Cooper (a maker of barrels, or a typo on copper Cu?  Cuprates?)
Grouper
Kuiper (yes, I know it's pronounced Kaiper)
Pooper
Scooper
Stupor
Trooper
Trouper
